Neural Predictive Monitoring under Partial Observability

We consider the problem of predictive monitoring (PM), i.e., predicting at runtime future violations of a system from the current state. We work under the most realistic settings where only partial and noisy observations of the state are available at runtime. Such settings directly affect the accuracy and reliability of the reachability predictions, jeopardizing the safety of the system. In this work, we present a learning-based method for PM that produces accurate and reliable reachability predictions despite partial observability (PO). We build on Neural Predictive Monitoring (NPM), a PM method that uses deep neural networks for approximating hybrid systems reachability, and extend it to the PO case. We propose and compare two solutions, an end-to-end approach, which directly operates on the rough observations, and a two-step approach, which introduces an intermediate state estimation step. Both solutions rely on conformal prediction to provide 1) probabilistic guarantees in the form of prediction regions and 2) sound estimates of predictive uncertainty. We use the latter to identify unreliable (and likely erroneous) predictions and to retrain and improve the monitors on these uncertain inputs (i.e., active learning). Our method results in highly accurate reachability predictions and error detection, as well as tight prediction regions with guaranteed coverage.

==> coverages_table.tex <==
\begin{table}
\centering
\begin{tabular}{ |c|r|r|r|r|r|r|r|r| }
\hline
&\multicolumn{7}{|c|}{original} \\
\hline
\textbf{Model} & \textbf{PO-NSC} & \textbf{Comb PO-NSC}& \textbf{NSC} & \textbf{NSE (box)}&\textbf{Eff (box)}& \textbf{NSE}&\textbf{Eff} \\
\hline
\textbf{SN} &94.84 & 94.68  & 94.68 & 97.04 & 0.34 & 94.69 &  1.373 \\
\textbf{IP} & 95.18 & 94.85 & 94.51& 97.24 & 6.64 & 94.65 & 3.064  \\
\textbf{CVDP} &95.78 & 95.63 & 95.64 & 98.55 & 0.0021 & 95.37 & 0.343 \\
\textbf{TWT} & 96.42 & 96.60 & 96.68 & 98.20 & 0.16818 & 95.07 & 0.770 \\
\textbf{LALO} & 94.84 & 94.66 & 94.88 & 99.03 & 0.00066 & 95.29 &  0.656\\
\textbf{HC} & 94.98 & 94.76 & 94.45 & 99.63 & $2.9\times 10^{15}$ & 94.39 & 12.401 \\
\textbf{AP} & 95.04 & 94.56 & 94.97 & 98.98 & 519.89 & 95.09 &  12.055 \\
\hline
\end{tabular}
\caption{Coverage and efficiency. Expected coverage $95\%$}
\begin{tabular}{ |c|r|r|r|r|r|r|r| }
\hline
&\multicolumn{7}{|c|}{active}\\
\hline
\textbf{Model} & \textbf{PO-NSC} & \textbf{Comb PO-NSC}& \textbf{NSC} & \textbf{NSE (box)}&\textbf{Eff (box)}& \textbf{NSE}&\textbf{Eff} \\
\hline
\textbf{SN} & 97.87 & 98.72 & 97.40 & 98.16 & 0.7691 & 94.60 & 1.361 \\
\textbf{IP} &  97.12 & 97.73 & 97.23  & 97.45 & 7.02 & 94.59 & 3.018 \\
\textbf{CVDP} & 97.89 & 98.31 & 98.25 & 98.70 & 0.0027 & 94.91 & 0.348 \\
\textbf{TWT} & 99.94 & 99.66 & 98.72 & 99.95 &  0.89968 & 95.15 & 0.825 \\
\textbf{LALO} &  97.37 & 97.48 & 98.01 & 98.90 &  0.002635 & 94.98 & 0.853 \\
\textbf{HC} & 97.56 &97.92 & 97.86 & 99.64 & $3.6\times 10^{15}$ & 94.44 & 12.401 \\
\textbf{AP} & 100.00 & 100.00 & 99.96 & 98.87 & 375.50 & 95.07 & 12.051 \\
\hline
\end{tabular}
\caption{Active. Coverage and efficiency. Expected coverage $95\%$}
\end{table}

==> cp.tex <==
\section{Methods}\label{sec:background}
In this section, we provide background on conformal prediction (CP) and explain how we apply this technique to endow our reachability predictions and state estimates with probabilistic guarantees. Then, we discuss how CP can be used to derive measures of predictive uncertainty to enable error detection and active learning. 

\np{double check that all notation is necessary, o/w remove} In the following, we present the methods assuming a generic prediction model. Let $X$ be the input space, $T$ be the target space, and define $Z = X\times T$. Let $\mathcal{Z}$ be the data-generating distribution, i.e., the distribution of the points $(x,t)\in Z$.  
The prediction model is represented as a function $f:X\rightarrow T$. 
For a generic input $x_i$ \np{not sure we need to keep indices $_i$ here}, we denote with $t_i$ the true target value of $x_i$ and with $\hat{t}_i$ the prediction by $f$. 
Test inputs, whose unknown true target values we aim to predict, are denoted by $x_*$.

In our setting of reachability prediction, inputs are observation sequences, target values are the corresponding reachability values. The data distribution $\mathcal{Z}$ is the joint distribution of observation sequences and  reachability values induced by state $s_{t-H_P}\sim \mathcal{S}$ and iid noise vector $\mathbf{w}_t$. 

\subsection{Conformal Prediction for regression and classification}

Conformal Prediction associates measures of reliability to any traditional supervised learning problem. It is a very general approach that can be applied across all existing classification and regression methods~\cite{balasubramanian2014conformal}. 
CP produces \textit{prediction regions with guaranteed validity}, thus satisfying the statistical guarantees illustrated in Problem~\ref{prbl:stat_guar}.

\begin{definition}[Prediction region]
For significance level $\varepsilon \in (0,1)$ and test input $x_*$, the $\varepsilon$-prediction region for $x_*$, $\Gamma_*^{\varepsilon}\subseteq T$, is a set of target values s.t.
\begin{equation}\label{eq:pred_r}
    \underset{(x_*,t_*)\sim \mathcal{Z}}{Pr}(t_* \in \Gamma_*^{\varepsilon}) = 1 - \epsilon.
\end{equation}
\end{definition}
%Thus, such a prediction region satisfies the statistical guarantees requirement of Problem~\ref{prbl:stat_guar}. In that case, the data-generating distribution $\mathcal{Z}$ is the joint distribution of observation sequences and corresponding reachability values induced by state $s_{t-H_P}\sim \mathcal{S}$ and iid noise vector $\mathbf{w}_t$.


%The CP algorithm outputs \textit{prediction regions}, instead of single point predictions: given a significance level $\varepsilon \in (0,1)$ and a test point $x_i$, its prediction region, $\Gamma_i^{\varepsilon}\subseteq T$, is a subset of $T$ guaranteed to contain the true value with probability $1 -\varepsilon$.

% The main ingredients of CP are: a \textit{nonconformity function} $\delta:Z \rightarrow \mathbb{R}$,  a set of
% labelled examples $Z'\subseteq Z$, 
% a classification model $f$ trained on a subset of $Z'$, 
% and a statistical test. The nonconformity function $\delta(z)$ measures the ``strangeness'' of an example $z_i=(x_i,t_i)$, i.e., the deviation between true value $t_i$ and the corresponding prediction $f(x_i)$. 



The idea of CP is to construct the prediction region by ``inverting'' a suitable hypothesis test: given a test point $x_*$ and a tentative target value $t'$, we \textit{exclude} $t'$ from the prediction region only if it is unlikely that $t'$ is the true value for $x_*$. The test statistic is given by a so-called \textit{nonconformity function (NCF)} $\ncf:Z \rightarrow \mathbb{R}$, which, given a predictor $f$ and a point $z=(x,t)$, measures the deviation between the true value $t$ and the corresponding prediction $f(x)$.  In this sense, $\ncf$ can be viewed as a generalized residual function. In other words, CP builds the prediction region $\Gamma_*^{\varepsilon}$ for a test point $x_*$ by excluding all targets $t'$ whose NCF values are unlikely to follow the NCF distribution of the true targets:
\begin{equation}\label{eq:cp_predr}
\Gamma_*^{\varepsilon} = \{t' \in T \mid  Pr_{(x,t)\sim \mathcal{Z}}(\ncf(x_*,t') \geq \ncf(x,t)) > \varepsilon\}.
\end{equation}
The probability term in Eq.~\ref{eq:cp_predr} is often called p-value. 
From a practical viewpoint, the NCF distribution $Pr_{(x,t)\sim \mathcal{Z}}(\ncf(x,t))$ cannot be derived in an analytical form, and thus we use an empirical approximation derived using a sample $Z_c$ of $\mathcal{Z}$.  This  approach is called \textit{inductive CP}~\cite{papadopoulos2008inductive} and $Z_c$ is referred to as \textit{calibration set}. 


\begin{remark}[Assumptions and guarantees of \np{inductive?} CP] Importantly, CP prediction regions have \textit{finite-sample validity} \np{cite}, i.e., they satisfy~\eqref{eq:pred_r} for any sample of $\mathcal{Z}$ (or reasonable size), and not just asymptotically. On the other hand, CP's theoretical guarantees hold under the \textit{exchangeability} assumption (a ``relaxed'' version of iid) by which the joint probability of any sample of $\mathcal{Z}$ is invariant to permutations of the sampled points. Of the two observation distributions discussed in Section~\ref{sec:problem}, we have that independent observations are exchangeable but sequential ones are not (due to the temporal dependency). Even though sequential data violate CP's theoretical validity, we find that the prediction regions still attain empirical coverage consistent with the nominal coverage (see results section), that is, the probabilistic guarantees still hold in practice (as also found in previous work on CP and time-series data \np{cite}).
\end{remark}


\subsubsection{CP for classification.} In classification, the target space is a discrete set of possible labels (or classes) $T=\{\ell^1,\ldots,\ell^c\}$.  We represent the classification model as a function $f:X\rightarrow [0,1]^c$ mapping inputs into a vector of class likelihoods, such that the predicted class is the one with the highest likelihood\footnote{Ties can be resolved by imposing an ordering over the classes.}. 
Classification is relevant for predictive monitoring as the reachability predictor of Problem~\ref{prbl:pm_po} is indeed a binary classifier ($T=\{0,1\}$) telling whether or not an unsafe state can be reached given a sequence of observation. 

The inductive CP algorithm for classification is divided into an offline phase, executed only once, and an online phase, executed for every test point $x_*$. In the offline phase (steps 1--3 below), we train the classifier $f$ and construct the calibration distribution, i.e., the empirical approximation of the NCF distribution. In the online phase (steps 4--5), we derive the prediction region for $x_*$ using said classifier and distribution.
\begin{enumerate}
    \item Draw sample $Z'$ of $\mathcal{Z}$. Split $Z'$ into training set $Z_t$ and calibration set $Z_c$.
    \item Train classifier $f$ using $Z_t$. Use $f$ to define an NCF $\delta$.
    \item Construct the calibration distribution by computing, for each $z_i \in Z_c$, the NCF score $\alpha_i = \delta(z_i)$.
    \item For each label $\ell^j \in T$, compute $\alpha_*^j = \delta(x_*,\ell^j)$, i.e., the NCF score for $x_*$ and $\ell^j$, and the associated p-value $p_*^{j}$:
    \begin{equation}\label{eq:smoothed_p}
p_*^{j}= \frac{|\{z_i\in Z_c \mid \alpha_i > \alpha_*^{j}\}|}{|Z_c|+1}+\theta\frac{|\{z_i\in Z_c \mid \alpha_i = \alpha_*^{j}\}|+1}{|Z_c|+1},
\end{equation}
where $\theta\in\mathcal{U}[0,1]$ is a tie-breaking random variable. 
\item Return the prediction region $\Gamma_*^{\varepsilon} = \{\ell^j\in T \mid p_*^{j}>\varepsilon\}.$
\end{enumerate}
In defining the NCF $\delta$, we should aim to obtain high $\delta$ values for wrong predictions and low $\delta$ values for correct ones. Thus, a natural choice in classification is to define $\delta(x,l^j) = 1 - f(x)_j$, where $f(x)_j$ is the likelihood predicted by $f$ for class $l_j$. Indeed, if $l^j$ is the true target for $x$ and $f$ correctly predicts $l^j$, then $f(x)_j$ is high (the highest among all classes) and $\delta(x,l^j)$ is low; the opposite holds if $f$ does not predict $l^j$.

% \subsection{CP for Classification}\label{sec:cp_class}

% In classification problems the target space is a discrete set of possible labels $T=\{\ell^1,\ldots,\ell^c\}$ be the set of labels (or classes).
% The classification model is represented as a function $f:X\rightarrow [0,1]^c$ mapping inputs into a vector of class likelihoods, such that the class predicted by $f$ corresponds to the class with the highest likelihood. 
% The prediction region, $\Gamma_i^{\varepsilon}\subseteq T$, is a set of labels guaranteed to contain the true label $\ell_i$ with probability $1 -\varepsilon$. 
% \subsubsection{CP algorithm for classification}

% Given a set of examples $Z'\subseteq Z$, a test input $x_*\in X$, and a significance level $\varepsilon\in [0,1]$,
% CP computes a prediction region $\Gamma_*^{\varepsilon}$ for $x_*$ as follows.
% \begin{itemize}
%     \item[1.] Divide $Z'$ into a training set $Z_{t}$, and calibration set $Z_{c}$. Let $q = |Z_{c}|$ be the size of the calibration set.

% \item[2.] Train a model $f$ using $Z_{t}$.
% \item[3.] Define a nonconformity function $\delta((x_i,\ell_i))=\Delta (f(x_i),\ell_i)$, i.e., choose a metric $\Delta$ to measure the distance between $f(x_i)$ and $\ell_i$ (see Section \ref{NCM}). 
% \item[4.] Apply $\delta (z)$ to each example $z$ in $Z_c$ and sort the resulting nonconformity scores $\{\alpha = \delta(z) \mid z \in Z_c\}$ in descending order: $\alpha_1\ge \cdots \ge\alpha_q$.
% \item[5.] Compute the nonconformity scores $\alpha_*^j = \delta((x_*,\ell^j))$ for the test input $x_*$ and each possible label $j\in \{1,\dots ,c\}$. Then, 
% compute the smoothed p-value
% \begin{equation}\label{eq:smoothed_p}
% p_*^{j}= \frac{|\{z_i\in Z_c : \alpha_i > \alpha_*^{j}\}|}{q+1}+\theta\frac{|\{z_i\in Z_c : \alpha_i = \alpha_*^{j}\}|+1}{q+1},
% \end{equation}
% where $\theta\in\mathcal{U}[0,1]$ is a tie-breaking random variable.  Note that $p_*^{j}$ represents the portion of calibration examples that are at least as nonconforming as the tentatively labelled test example $(x_*, \ell^j)$. 
% \item[6.] Return the prediction region  
% \begin{equation}
% \Gamma_*^{\varepsilon} = \{\ell^j\in L : p_*^{j}>\varepsilon\}.
% \end{equation}
% together with a vector of p-values, one for each class.
% \end{itemize}
% Note that in this approach, called inductive CP \cite{papadopoulos2008inductive}, steps 1--4 are performed only once, while Steps 5--6 are performed for every test point $x_*$.


% \paragraph{Nonconformity function.}
% A nonconformity function is well-defined if it assigns low scores to correct predictions and high scores to wrong predictions. A natural choice for $\delta$, based on the underlying model $f$, is $f(z) = \Delta (f(x_i),\ell_i)$, where 
% $\Delta$ is a suitable distance\footnote{The choice of $\Delta$ is not very important, as long as it is symmetric.}.
% Recall that, for an input $x \in X$, the output of $f$ is a vector of class likelihoods, which we denote by $f(x) = [P_f(\ell_1|x), \ldots, P_f(\ell_c|x)]$. In classification problems, a common well-defined nonconformity function is obtained by defining $\Delta$ as
% \begin{equation}\label{std_NCM}
% \Delta (f(x_i),\ell_i)=1-P_{f}(\ell_i|x_i), 
% \end{equation}
% where $P_{f}(\ell_i|x_i)$ is the likelihood of class $\ell_i$ when the model $f$ is applied on $\ell_i$. If $f$ correctly predicts $\ell_i$ for input $x_i$, the corresponding likelihood $P_{f}(\ell_i|x_i)$ is high (the highest among all classes) and the resulting nonconformity score is low. The opposite holds when $f$ does not predict $\ell_i$. The nonconformity measure chosen for our experiments, Equation~\ref{std_NCM}, preserves the ordering of the class likelihoods predicted by $f$.


\subsubsection{CP for Regression.}\label{sec:cp_regr}
\np{I thought we should not use $y$ for the inputs below, but keep the generic $x$ notation}
In regression we have a continuous target space $T\subseteq\mathbb{R}^n$. Thus, the regression case is relevant for us because our state estimator can be viewed as a regression model, where $T$ is the state space. 

The CP algorithm for regression is similar to the classification one. In particular, the offline phase of steps 1--3, i.e., training of regression model $f$ and definition of NCF $\delta$, is the same (with obviously a different kind of $f$ and $\delta$). 

The online phase changes though, because $T$ is a continuous space and thus, it is not possible to enumerate the target values and compute for each a p-value. Instead, we proceed in an equivalent manner, that is, identify the critical value $\alpha_{(\varepsilon)}$ of the calibration distribution, i.e., the NCF score corresponding to a p-value of $\varepsilon$. The resulting $\varepsilon$-prediction region is given by $\Gamma_*^{\varepsilon} = f(x_*) \pm \alpha_{(\varepsilon)}$, where $\alpha_{(\varepsilon)}$ is the $(1-\varepsilon)$-quantile of the calibration distribution, i.e., the $\lfloor \varepsilon \cdot (|Z_c|+1)\rfloor$-th largest calibration score. 

In the algorithm above, each prediction interval has the same width. Some more advanced approaches to CP regression allow to obtain prediction regions with varying interval width. For instance, one can define a normalized nonconformity function or resort to conformalized quantile regression~\cite{romano2019conformalized}. The application of such methods is not straightforward and thus, in this work, we limit prediction regions to have constant width.

% Let $Y$ be the input space, $T\subseteq\mathbb{R}^n$ be the target space, and define $Z = Y\times T$.
% The regression model is represented as a function $f:Y\rightarrow T$. For a generic input $y_i$, we  denote  with $t_i$ the real target value associated to it.

\paragraph{Nonconformity score.} The target space is a $n$-dimensional space, a proper nonconformity measure could be the norm of the difference among the real and the predicted vector. This is the NCS used in our experiments for the regression tasks. Another possible choice is to consider $n$ different scores, one for each variable, so that we are able to provide statistical guarantees about the quality of the reconstruction on a variable-specific basis. 




% \subsubsection{CP algorithm for regression}

% The first steps of the algorithm, from 1 to 4, are similar to the ones of the classification algorithm. Given a set of examples $Z'\subseteq Z$, a test input $x_*\in X$, and a significance level $\varepsilon\in [0,1]$,

% \begin{itemize}
%     \item[1.] Divide $Z'$ into a training set $Z_{t}$, and calibration set $Z_{c}$. Let $q = |Z_{c}|$ be the size of the calibration set.
% \item[2.] Train a model $f$ using $Z_{t}$.
% \item[3.] Define a nonconformity function $\delta(z_i)=\Delta (f(x_i),t_i)$, i.e., choose a metric $\Delta$ to measure the distance between $f(x_i)$ and $t_i$. 
% \item[4.] Apply $\delta (z)$ to each example $z$ in $Z_c$ and sort the resulting nonconformity scores $\{\alpha = \delta(z) \mid z \in Z_c\}$ in descending order: $\alpha_1\ge \cdots \ge\alpha_q$.
% \item[5.] Compute $\alpha_{\tau}$, which is the $(1-\epsilon)$-percentile nonconformity score. The prediction region for a new example $x_*$ is $\Gamma_*^{\epsilon} = f(x_*) \pm \alpha_{\tau}$
% \end{itemize}
% The prediction region $\Gamma_*^{\epsilon} $ contains the real target value with probability $1-\epsilon$.



\subsubsection{Validity and Efficiency}
CP performances are measured via two quantities: \emph{validity} (or \emph{coverage}), i.e. the coherence between $\epsilon$ and the error rate, and 
the \emph{efficiency}, i.e. the size of the prediction regions. CPs are automatically valid, whereas the efficiency depends on the chosen nonconformity function and thus the underlying model.


\np{move conf and cred into the uncertainty measures section} 
\subsubsection{Confidence and credibility}\label{sec:conf_cred}
Observe that, for significance levels  $\varepsilon_1\ge\varepsilon_2$, the corresponding prediction regions are such that $\Gamma^{\varepsilon_1}\subseteq \Gamma^{\varepsilon_2}$.  
It follows that, given an input $x_*$, if $\varepsilon$ is lower than all its p-values, i.e. $\varepsilon < \min_{j=1,\ldots,c} \ p_*^{j}$, then the region $\Gamma_*^{\varepsilon}$ contains all the labels. As $\varepsilon$ increases, fewer and fewer classes will have a p-value higher than $\varepsilon$. That is, the region shrinks as $\varepsilon$ increases. In particular, $\Gamma_*^{\varepsilon}$ is empty when $\varepsilon \geq \max_{j=1,\ldots,c} \ p_*^{j}$.  

The \textit{confidence} of a point $x_*\in X$, $1-\gamma_*$, measures how likely is our prediction for $x_*$ compared to all other possible classifications (according to the calibration set). It is computed as one minus the smallest value of $\varepsilon$ for which the conformal region is a single label, i.e. the second largest p-value $\gamma_*$: 
\[1-\gamma_* = \sup \{1-\varepsilon : |\Gamma_*^{\varepsilon}| = 1\}.\]

The \textit{credibility}, $c_*$, indicates how suitable the training data are to classify that specific example. In practice, it is the smallest $\varepsilon$ for which the prediction region is empty, i.e. the highest p-value according to the calibration set, which corresponds to the p-value of the predicted class: 
\[c_* = \inf \{\varepsilon : |\Gamma_*^{\varepsilon}|= 0\}.\]


Note that if $\gamma_*\le \varepsilon$, then the corresponding prediction region $\Gamma_*^{\varepsilon}$ contains at most one class. If both $\gamma_*\le \varepsilon$ and $c_* > \varepsilon$ hold, then the prediction region contains \textit{exactly} one class, i.e., the one predicted by $f$. In other words, the interval $[\gamma_*, c_*)$ contains all the $\varepsilon$ values for which we are sure that $\Gamma_*^{\varepsilon}=\{\hat{\ell}_*\}$. 
It follows that the higher $1-\gamma_*$ and $c_*$ are, the more reliable the prediction $\hat{\ell}_*$ is, because we have an expanded range $[\gamma_*, c_*)$ of significance values by which $\hat{\ell}_*$ is valid. 
Indeed, in the extreme scenario where $c_*=1$ and $\gamma_*=0$, then $\Gamma_*^{\varepsilon}=\{\hat{\ell}_*\}$ for any value of $\epsilon$. This is why, as we will explain in the next section, our uncertainty-based rejection criterion relies on excluding points with low values of $1-\gamma_*$ and $c_*$. We stress, in particular, the following statistical guarantee: 
the probability that the true prediction for $x_*$ is exactly $\hat{\ell}_*$ is at most $1-\gamma_*$. 

In binary classification problems, each point $x_*$ has only two p-values, one for each class, which coincide with $c_*$ (p-value of the predicted class) and $\gamma_*$ (p-value of the other class). 





==> methods.tex <==
\section{Methods}\label{sec:methods}
%\np{how about a structure like below?
%\begin{itemize}
%    \item subsection on CP -- see also text in the STTT paper;
%    explain assumptions and guarantees (discuss theoretical validity and empirical coverage for independent vs sequential observation assumptions); briefly present algorithms for classification and for regression
%    \item subsection on end-to-end PM, including presentation of learning solution (dataset generation+classifier training), choice of NCF
%    \item subsection on two-step PM, including presentation of learning solution (dataset generation+regressor training+joint training with reachability predictor)+choice of NCF+prediction regions with Bonferroni
%    \item uncertainty measures and optimal rejection rule
%    \item active learning algorithm; discuss dataset shift and theoretical+practical implications on validity
%\end{itemize}
%}


\subsection{Dataset Generation}\label{sec:data_gen}
The key component of NPM is to express PM as a supervised learning problem, which calls for the generation of a dataset used suitable to learn the approximate reachability predictor. The rationale is to use traditional reachability checkers to label states $s$ as safe, if $\mathcal{M}\models \mathsf{Reach}(U,s,H_f)$, or unsafe. The reachability of the system at time $t$ only on the state of the system at time $t$, however, one can decide to make a prediction based on the sequence $\mathbf{s}_t$ of the previous $H_p$ states, $\mathbf{s}_t = s_{t-H_p}\cdots s_t$. Formally, the dataset can be expressed as $\mathcal{D}_{NPM} = \{(\mathbf{s}^{i}, l_i)\}_{i=1}^N$, where $\mathbf{s}^i = (s^i_{t-H_p},s^i_{t-H_p+1},\dots, s^i_t)$ and $l_i = \mathbf{1}(\mathsf{Reach}(U,s^i_t,H_f))$ for a generic $t$.
Under PO, we assume that the measurement process can be modeled by a function $\mu:S\rightarrow Y$, which is then used to form a dataset $\mathcal{D}_{PO-NPM}$ made of tuples $(\mathbf{y}_t, \mathbf{s}_t, l_t)$, where $\mathbf{y}_t$ is a noisy observation of $\mathbf{s}_t$, i.e. a sequence of length $H_p$ such that $y_{j} = \mu(s_j)+w_j$, for $w_j\sim\mathcal{W}$ and $\forall j\in\{t-H_p,\dots , t\}$.
The data generating distribution $\mathcal{S}$ determines how states $\mathbf{s}_t$ are sampled. In our experiments, we consider the \emph{independent} scenario, in which each state, and thus its history, is sampled independently from all the other states, and the \emph{sequential} scenario in which states (and their history) comes from temporally correlated trajectories in a sliding-window fashion. The latter is more suitable for real runtime applications. On the other hand, we loose the property of exchangeability, which is a fundamental requirement for CP to guarantee validity.

\subsection{NPM under PO}
Two alternative approaches (as introduced in Section~\ref{sec:pm_po}) can be considered starting from $\mathcal{D}_{PO-NPM}$ to solve Problem~\ref{prbl:pm_po}:

\begin{enumerate}
\item \textbf{End-to-end}: we train a CNN that learns a direct mapping from $\mathbf{y}_t$ to $l_t$, which becomes a simple binary classification problem. This approach ignores the sequence of states $\mathbf{s}_t$. The loss function is the canonical cross-entropy typically used in binary classification problems.
    
\item \textbf{Two-step}: we train in parallel a CNN regressor, referred to as Neural State Estimator (NSE), to reconstruct the sequence of states $\hat{\mathbf{s}}_t$ from the series of noisy observations $\mathbf{y}_t$, and a CNN classifier referred to as Neural State Classifier (NSC), that predicts the safety label $l_t$ from the sequence of states $\mathbf{s}_t$. The combination of the two CNN, the NSE and the NSC maps the sequence of noisy measurements into the safety label, as required in Problem~\ref{prbl:pm_po}. However, the NSE inevitably introduces some errors in the reconstruction $\hat{\mathbf{s}}_t$ of $\mathbf{s}_t$. Such error is propagated by evaluating NSC on $\hat{\mathbf{s}}_t$, causing a low accuracy of the combined net. 
To improve the performances of the combined function, we perform a \emph{fine-tuning} step in which the weights of the NSE and the weights of the NSC are updated together via the minimization of a loss that combines the two respective losses. In this step, the NSC learn to classify correctly the state reconstructed by the NSE, $\hat{\mathbf{s}}_t$, rather than the real state $\mathbf{s}_t$, so to improve the task specific accuracy. It is likely that such fine-tuning will lower the performances of the exact states, but this problem does not concern us, since under PO exact states are not available at test time. 
The loss for the NSE is the mean square error among the real sequences of states $\mathbf{s}_t$ and the reconstructed ones $\hat{\mathbf{s}}_t$, whereas for the NSC we use, once again a binary cross-entropy loss. 
\end{enumerate}

\subsubsection{Neural State Estimation}
Two-step approach has an important collateral advantage, which is the NSE. In general, any state of the art state estimator can be used here. However, we are dealing with complex non-linear systems. The black-box NSE reaches very high reconstruction precision and furthermore, because of the fine-tuning and potentially active learning, we can calibrate the estimates to be more accurate in safety critical regions. 




==> table.tex <==
\begin{table}
\centering
\begin{tabular}{ |c|r|r|r|r|r||r|r|r|r|r| }
\hline
&\multicolumn{5}{|c|}{original} & \multicolumn{5}{|c|}{active}\\
\hline
\textbf{Model} & \textbf{Acc.} & \textbf{Det.} & \textbf{FN}&\textbf{FP}& \textbf{Rej.} &\textbf{Acc.} & \textbf{Det.} & \textbf{FN}&\textbf{FP} & \textbf{Rej.} \\
\hline
\textbf{SN} & 97.75 & 98.67 & 67/67 & 155/158 & 11.88 & 97.65 & 98.30 & 51/52 & 180/183 & 14.06 \\
\textbf{IP} & 99.01 & 95.96 & 38/40 & 57/59 & 6.78 & 99.13 & 94.25 & 41/43 & 41/44 & 5.32\\
\textbf{CVDP} & 99.68 & 100.00 &17/17 & 15/15 & 3.51 & 99.69 & 100.00 & 19/19 & 12/12 & 2.48 \\
\textbf{TWT} & 98.93 & 96.26 & 52/56 & 51/51 & 10.46 & 99.07 & 94.62 & 44/49 & 44/44 & 6.20\\
\textbf{LALO} & 99.24 & 100.00 & 52/52  & 24/24 & 6.11 & 99.27 &100.00& 40/40 & 33/33 & 4.28 \\
\textbf{HC} & 99.80 & 100.00 & 10/10 & 10/19 &4.02 & 99.84 & 100.00 & 11/11 & 5/5 & 2.40 \\
\textbf{AP} & 99.26 & 100.00 & 48/48 & 26/26 & 5.79 &99.41  & 100.00 & 19/19 & 40/40 & 20.77 \\
\hline
\end{tabular}
\caption{Two steps approach.}
\end{table}

\begin{table}
\centering
\begin{tabular}{ |c|r|r|r|r|r||r|r|r|r|r| }
\hline
&\multicolumn{5}{|c|}{original} & \multicolumn{5}{|c|}{active}\\
\hline
\textbf{Model} & \textbf{Acc.} & \textbf{Det. }&\textbf{FN}&\textbf{FP} & \textbf{Rej.} &\textbf{Acc.} & \textbf{Det.} &\textbf{FN}&\textbf{FP} & \textbf{Rej.} \\
\hline
\textbf{SN} & 97.75 & 98.67 & 67/67 & 155/158 & 11.88 & 97.65 & 98.30 & 51/52 & 180/183 & 14.06 \\
\textbf{IP} & 95.78 & 86.95 & 168/194  & 203/248&20.03 & 95.22 & 88.07 & 249/270 & 172/208 & 26.26\\
\textbf{CVDP} & 99.19 & 100.00 &30/30 & 51/51 & 5.75 & 99.10 & 95.55 & 43/46 & 43/44 & 4.81 \\
\textbf{TWT} & 98.93 & 95.51 & 18/20 & 67/69 & 7.45 & 99.04 & 100.00 & 45/45 & 62/62 & 10.45 \\
\textbf{LALO} & 98.88 & 99.11 & 66/66 & 45/46 & 7.39 & 98.79 & 96.69 &87/90 & 30/31 & 6.88  \\
\textbf{HC} & 99.68 & 100.00 & 18/18 & 16/16 & 4.75 & 99.64 & 100.00 & 17/17 & 20/20 & 3.31 \\
\textbf{AP} & 96.35 & 93.15 & 167/185 & 173/180 & 19.59 & 96.53 & 99.42 & 137/139 & 208/208  &  35.05\\
\hline
\end{tabular}
\caption{One steps approach.}
\end{table}

\begin{table}
\centering
\begin{tabular}{ |c|r|r|r||r|r|r| }
\hline
&\multicolumn{3}{|c|}{original} & \multicolumn{3}{|c|}{active}\\
\hline
\textbf{Model} & \textbf{NSC Acc.} & \textbf{PO-NSC Acc}&\textbf{Comb. PO-NSC Acc.}&\textbf{NSC Acc.} & \textbf{PO-NSC Acc}&\textbf{Comb. PO-NSC Acc.} \\
\hline
\textbf{SN} & 96.44 & 98.17 & 98.52 & 93.56 & 98.31 & 98.51   \\
\textbf{IP} & 94.32 & 92.03 & 99.01 & 93.14 & 95.93 & 99.13 \\
\textbf{CVDP} &99.59 & 99.53 & 99.68 & 99.54 & 99.51 & 99.69 \\
\textbf{TWT} & 96.75 & 99.13 & 99.07 & 98.70 & 99.23 & 98.93   \\
\textbf{LALO} & 95.77  & 98.54 & 99.23  & 88.84 & 98.00 & 99.26 \\
\textbf{HC} & 98.71 & 99.81 & 99.80 & 98.24 & 99.78 & 99.84 \\
\textbf{AP} & 95.02 & 96.33 & 99.26 & 97.39 & 96.56 & 99.41 \\
\hline
\end{tabular}
\caption{Comparing the accuracies.}
\end{table}
